Stochastic Gradient Methods with Compressed Communication for Decentralized Saddle Point Problems

We develop two compression based stochastic gradient algorithms to solve a class of non-smooth strongly convex-strongly concave saddle-point problems in a decentralized setting (without a central server). Our first algorithm is a Restart-based Decentralized Proximal Stochastic Gradient method with Compression (C-RDPSG) for general stochastic settings. We provide rigorous theoretical guarantees of C-RDPSG with gradient computation complexity and communication complexity of order $\mathcal{O}( (1+\delta)^4 \frac{1}{L^2}{\kappa_f^2}\kappa_g^2 \frac{1}{\epsilon} )$, to achieve an $\epsilon$-accurate saddle-point solution, where $\delta$ denotes the compression factor, $\kappa_f$ and $\kappa_g$ denote respectively the condition numbers of objective function and communication graph, and $L$ denotes the smoothness parameter of the smooth part of the objective function. Next, we present a Decentralized Proximal Stochastic Variance Reduced Gradient algorithm with Compression (C-DPSVRG) for finite sum setting which exhibits gradient computation complexity and communication complexity of order $\mathcal{O} \left((1+\delta) \max \{\kappa_f^2, \sqrt{\delta}\kappa^2_f\kappa_g,\kappa_g \} \log\left(\frac{1}{\epsilon}\right) \right)$. Extensive numerical experiments show competitive performance of the proposed algorithms and provide support to the theoretical results obtained.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%In a single machine setting, stochastic variance reduced gradient (SVRG) methods have been developed for saddle point problems with a specific bilinear structure \cite{balamuruganbach2016svrgsaddle}, and stochastic primal dual methods with a restart scheme are available for saddle point problems without a bilinear structure \cite{yanetal2019stocprimaldual}.   

%\textbf{Decentralized minimization:} We provide here only a very brief survey of literature on decentralized minimization (see \textit{e.g.} \cite{li2021decentralized} for more comprehensive survey). A simple distributed deterministic gradient method with sublinear convergence rate guarantees was proposed in \cite{ram2009distributed}. Distributed gradient methods using gradient tracking \cite{extra2015shietal, pu2020push} are known to converge to an exact optimal value using constant step size. Stochastic gradient oracles for decentralized minimization problems proposed in \cite{Mokhtari2016DSADD}, have recently been extended to design efficient compression based decentralized methods for solving convex minimization problems with provable theoretical guarantees \cite{koloskova2019decentralized,liu2020linear,li2021decentralized}. More recent works are proposed for non-convex optimization in decentralized settings \cite{xinetal2021decentralizednoncvx}. 
%
%\textbf{Decentralized saddle-point problems:}  
%\textbf{Decentralized minimization:}  Several existing works address decentralized convex minimization: e.g. distributed gradient methods \cite{ram2009distributed}, gradient tracking methods \cite{extra2015shietal, pu2020push}, stochastic gradient oracle (SGO) based  methods \cite{Mokhtari2016DSADD}, SGO+compression based methods \cite{koloskova2019decentralized,liu2020linear,li2021decentralized}; see \cite{li2021decentralized} for detailed survey. Recent works focus on non-convex optimization in decentralized settings \cite{xinetal2021decentralizednoncvx}. 

\setlength\arrayrulewidth{1pt}
\begin{table}[ht!]
	\setlength{\tabcolsep}{1pt}
	\caption{Comparison of proposed optimization algorithms for decentralized saddle point problems with state-of-the-art algorithms. SG denotes Stochastic Gradient. Abbreviations SC-SC, C-C, NC-NC respectively stands for Strongly convex-Strongly concave, Convex-Concave, Nonconvex-Nonconcave. GSS and FSS stands respectively for general stochastic setting and finite sum setting  } 	\label{ratetable}
%	\vspace{-0.1in}
%	\begin{center} 
	\centering
		\begin{tabular}{|cc|c|c|c|c|c|c|}
			\hline
			\multicolumn{2}{|l|}{}  & \textbf{Algorithm} &  \textbf{SG} &  \textbf{Non-} &  \textbf{Type of } & \textbf{Computation} & \textbf{Communication}  \\
			\multicolumn{2}{|l|}{} &  &  &   \textbf{smooth} &  \textbf{functions} & \textbf{Complexity} & \textbf{Complexity}  \\ \hhline{|-|-|-|-|-|-|-|-|}
			\multicolumn{1}{|c|}{\multirow{12}{*}{ \rotatebox{90}{\textbf{No compression}} }} & \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Gossip}}}} &  MMDS \cite{beznosikovetal2020distsaddle}  &  \xmark & \xmark &  \cellcolor[HTML]{FFCB2F} SC-SC &  $-$ &  $\tilde{\mathcal{O}}( \log^2(\frac{1}{\epsilon}) )$  \\ \hhline{|~|~|-|-|-|-|-|-|}
			%		\multicolumn{1}{|l|}{} &   & MMDS \cite{beznosikovetal2020distsaddle}  & \xmark &  \xmark & \xmark & SC-SC & $\textemdash$ & $\tilde{\mathcal{O}}( \log^2(\frac{1}{\epsilon}) )$  \\ \cline{3-9} 
			\multicolumn{1}{|l|}{} &  &  DES \cite{beznosikov2020distributed} & \cmark  &  \xmark & \cellcolor[HTML]{FFCB2F} SC-SC & $\tilde{\mathcal{O}}( \frac{\kappa_f^2}{L^2\epsilon} )$ & $\tilde{\mathcal{O}}( \kappa_f \sqrt{\kappa}_g \log(1/\epsilon ) )$  \\ \hhline{|~|~|-|-|-|-|-|-|}
			\multicolumn{1}{|l|}{} &  & Algorithm 1+3 \cite{kovalev2022optimal}  & \cmark & \cmark & \cellcolor[HTML]{FFCB2F} SC-SC  & $\mathcal{O}\left(\kappa_f \log(1/\epsilon ) \right)$  & $\mathcal{O}\left(\kappa_f \sqrt{\kappa_g} \log(1/\epsilon ) \right)$ \\ \cline{3-8}
			\multicolumn{1}{|l|}{} &  &  DPOSG \cite{liu2020decentralized} & \cmark & \xmark & NC-NC & $\mathcal{O}(\frac{1}{\epsilon^{12}})$ & $\tilde{\mathcal{O}}( \frac{1}{\epsilon^{12}} )$ \\ \hhline{|~|-|-|-|-|-|-|-|} 
			\multicolumn{1}{|l|}{} & \multirow{8}{*}{ \rotatebox{90}{\textbf{No Gossip} } } &  GT-EG \cite{mukherjeecharaborty2020decentralizedsaddle} & \xmark & \xmark & \cellcolor[HTML]{FFCB2F} SC-SC & $\mathcal{O}\left(\kappa_f^{4/3} \kappa_g^{4/3} \log\left(\frac{1}{\epsilon} \right)\right)$ & $\mathcal{O}\left(\kappa_f^{4/3} \kappa_g^{4/3} \log\left(\frac{1}{\epsilon} \right)\right)$  \\ \hhline{|~|~|-|-|-|-|-|-|} 
			\multicolumn{1}{|l|}{} &  & DSPAwLA\cite{nunezcortes2017distsaddlesubgrad}  & \xmark & \cmark & C-C & $\mathcal{O}(1/\epsilon^2)$ & $\mathcal{O}(1/\epsilon^2)$  \\ \cline{3-8} 
			\multicolumn{1}{|l|}{} &  &   DMHSGD \cite{xianetal2021fasterdecentnoncvxsp} & \cmark & \xmark & NC-SC & $\mathcal{O}(\frac{\kappa^3}{(1-\lambda_2(W))^2\epsilon^{3}} )$ & $\mathcal{O}(\frac{\kappa^3}{(1-\lambda_2(W))^2\epsilon^{3}} )$  \\ \hhline{|~|~|-|-|-|-|-|-|}
			\multicolumn{1}{|l|}{} &  & {\color{blue}{C-RDPSG}} & \cmark & \cmark & \cellcolor[HTML]{FFCB2F} &  &   \\
			\multicolumn{1}{|l|}{} &  &  \textbf{(Theorem \ref{thm:complexity_general_stoch})} & & & \cellcolor[HTML]{FFCB2F} SC-SC  & $\mathcal{O}(\frac{\kappa_f^2 \kappa^2_g}{L^2\epsilon} )$ & $\mathcal{O}(\frac{\kappa_f^2 \kappa^2_g}{L^2\epsilon} )$ \\
			\multicolumn{1}{|l|}{} &  &  \textbf{(GSS)} & & & \cellcolor[HTML]{FFCB2F}  & & \\ \hhline{|~|~|-|-|-|-|-|-|}
			\multicolumn{1}{|l|}{} &  &  {\color{blue}{C-DPSVRG}}  & \cmark &  \cmark & \cellcolor[HTML]{FFCB2F} & $\mathcal{O}(\max \{\kappa_f^2, \kappa_g \} $ & $\mathcal{O}(\max \{\kappa_f^2, \kappa_g \} $  \\ 
			\multicolumn{1}{|l|}{} &  &  \textbf{(Theorem \ref{thm:svrg_complexity})} & & & \cellcolor[HTML]{FFCB2F} SC-SC & $ \hspace*{0.3cm} \log( \frac{1}{\epsilon} ) )$ & $ \hspace*{0.3cm} \log( \frac{1}{\epsilon} ) )$ \\ 
			\multicolumn{1}{|l|}{} &  &  \textbf{(FSS)} & & & \cellcolor[HTML]{FFCB2F} &  &  \\ \hline \hline
			%		\multicolumn{1}{|l|}{} &  & (\textbf{FSS}) & & & {\cellcolor[HTML]{FFCB2F}} &  & \hline \hline
			%	\multicolumn{1}{|c|}{\multirow{4}{*}{ \rotatebox{90}{\textbf{Compression}}}} & \multirow{1}{*}{\rotatebox{90}{\textbf{Gossip}}} & - & - & - & - & - & -  \\ \cline{2-8} 
			%	& & & & & &  & \\ \cline{2-8} 
			\multicolumn{1}{|c|}{\multirow{4}{*}{ \rotatebox{90}{\textbf{Compression}}}} & \multirow{4}{*}{\rotatebox{90}{\textbf{No Gossip}}} &  {\color{blue}{C-RDPSG}} & \cmark & \cmark & \cellcolor[HTML]{FFCB2F}  &  &  \\ 
			\multicolumn{1}{|l|}{} &  &  \textbf{(Theorem \ref{thm:complexity_general_stoch})} & & & \cellcolor[HTML]{FFCB2F} SC-SC & $\mathcal{O}(\frac{(1+\delta)^4\kappa_f^2 \kappa^2_g}{L^2\epsilon} )$ & $\mathcal{O}(\frac{(1+\delta)^4\kappa_f^2 \kappa^2_g}{\epsilon} )$  \\
			\multicolumn{1}{|l|}{} &  &  \textbf{(GSS)} & & & \cellcolor[HTML]{FFCB2F}  & & \\ \hhline{|~|~|-|-|-|-|-|-|} 
			\multicolumn{1}{|l|}{} &  & {\color{blue}{C-DPSVRG}} & \cmark &  \cmark & \cellcolor[HTML]{FFCB2F} & $\mathcal{O}((1+\delta) $ & $\mathcal{O}((1+\delta)$  \\ 
			\multicolumn{1}{|l|}{} &  &  \textbf{(Theorem \ref{thm:svrg_complexity})} &  & & \cellcolor[HTML]{FFCB2F} SC-SC & $ \max \{\kappa_f^2, \sqrt{\delta}\kappa^2_f\kappa_g,\kappa_g \} )$ & $ \max \{\kappa_f^2, \sqrt{\delta}\kappa^2_f\kappa_g,\kappa_g \}  )$  \\ 
			\multicolumn{1}{|l|}{} &  & (\textbf{FSS}) & & & \cellcolor[HTML]{FFCB2F} & $ \hspace*{0.3cm}  \log( \frac{1}{\epsilon} ) )$ & $ \hspace*{0.3cm} \log( \frac{1}{\epsilon} ) )$  \\ \hline
		\end{tabular}
%	\end{center}
\end{table}
\setlength\arrayrulewidth{0.4pt} 

\textbf{Decentralized saddle-point problems:} A distributed saddle-point algorithm with Laplacian averaging (DSPAwLA) in \cite{nunezcortes2017distsaddlesubgrad}, based on gradient descent ascent updates to solve non-smooth convex-concave saddle point problems achieves $\mathcal{O}(1/\epsilon^2)$ convergence rate. \red{ DSPAwLA uses consensus constrained formulation of saddle point problem. DSPAwLA  is obtained by incorporating $\ell_2$ norm based penalty of consensus constraints into the objective function and employing gradient descent ascent scheme to the resultant penalized objective. However, our work proposes an equivalent Lagrangian formulation of consensus constrained saddle point problem \eqref{eq:main_opt_consenus_constraint} and updates primal-dual variables using a variant of primal dual hybrid method.} An extragradient method with gradient tracking (GT-EG) proposed in \cite{mukherjeecharaborty2020decentralizedsaddle} is shown to have linear convergence rates for solving decentralized strongly convex strongly concave problems, under a positive lower bound assumption on the gradient difference norm. However such assumptions might not hold for problems without bilinear structure. \red{Both \cite{mukherjeecharaborty2020decentralizedsaddle} and \cite{nunezcortes2017distsaddlesubgrad} are based on non-compression communications and full batch gradient computations which limit their applicability to large scale machine learning problems.} Recently, multiple works \cite{liu2020decentralized,xianetal2021fasterdecentnoncvxsp, beznosikov2020distributed} have proposed using minibatch gradients for solving decentralized saddle point problems. Decentralized extra step (DES) \cite{beznosikov2020distributed} shows linear  communication complexity with dependence on the graph condition number as $\sqrt{\kappa_g}$,   obtained at the cost of incorporating multiple rounds of communication of primal and dual updates. A near optimal distributed Min-Max data similarity (MMDS) algorithm is proposed in \cite{beznosikovetal2020distsaddle} for saddle point problems with a suitable data similarity assumption. MMDS is based on full batch gradient computations and requires solving an inner saddle point problem at every iteration. MMDS allows for communication efficiency by choosing only one node uniformly at random to update the iterates. However, every node computes the full batch gradient before heading to next gradient based updates. Moreover, this scheme employs accelerated gossip \cite{liu2011accelerated} multiple times to propagate the gradients and model updates to the entire network. Communication complexity of MMDS is shown to depend on eigengap of weight matrix $W$, while gradient computation complexity is not investigated.
%Multiple full-batch gradient computations and multiple rounds of communications requires a lot of time to finish even a single iterate. 
Decentralized parallel optimistic stochastic gradient method (DPOSG) was proposed in \cite{liu2020decentralized} for nonconvex-nonconcave saddle point problems. This method involves local model averaging step (multiple communication rounds) to reduce the effect of consensus error. A gradient tracking based algorithm called DMHSGD for solving nonconvex-strongly concave saddle point problems proposed in \cite{xianetal2021fasterdecentnoncvxsp}, uses a large mini-batch at the first iteration and requires the nodes to communicate both model and gradient updates, to achieve better aggregates of quantities. Variance reduction based optimal methods to solve strongly convex-strongly concave nonsmooth finite sum variational inequalities are developed in \red{\cite{kovalev2022optimal}. The improvement of complexity on graph condition number $\kappa_g$ in \cite{kovalev2022optimal} is achieved using an accelerated gossip scheme. However, C-DPSVRG does not involve any gossip scheme and hence yields cheaper communication per iterate. The complexity of C-DPSVRG and C-RDPSG does not have optimal dependence on $\kappa_f$, $\kappa_g$ and we leave it as a future work. } Table \ref{ratetable} positions our work in the context of existing methods. 

%\resizeableyellownote{2.5}{2.2}{In the extension version, add some experimental results for AUC over hetrogenous data sets.}  

 
%\textbf{Decentralized saddle-point problems:} A distributed saddle-point algorithm with Laplacian averaging (DSPAwLA) in \cite{nunezcortes2017distsaddlesubgrad}, based on gradient descent ascent updates to solve non-smooth convex-concave saddle point problems achieves $\mathcal{O}(1/\epsilon^2)$ convergence rate. An extragradient method with gradient tracking (GT-EG) proposed in \cite{mukherjeecharaborty2020decentralizedsaddle} is shown to have linear convergence rates for solving decentralized strongly convex strongly concave problems, under a positive lower bound assumption on the gradient difference norm. 
%%However such assumptions might not hold for problems without bilinear structure, and 
%The dependence of rates in \cite{mukherjeecharaborty2020decentralizedsaddle} on condition number $\kappa_g$ is unknown. 
%%Both \cite{mukherjeecharaborty2020decentralizedsaddle} and \cite{nunezcortes2017distsaddlesubgrad} do not consider compression and are based on full batch gradient computations. 
%Recently, multiple works \cite{liu2020decentralized,xianetal2021fasterdecentnoncvxsp, beznosikov2020distributed} have proposed using minibatch gradients for solving decentralized saddle point problems. Decentralized extra step (DES) \cite{beznosikov2020distributed} shows linear  communication complexity with dependence on the graph condition number as $\sqrt{\kappa_g}$,   obtained at the cost of incorporating multiple rounds of communication of primal and dual updates. 
%%The dependence of computation cost of DES on $\kappa_g$ is however not made explicit in \cite{beznosikov2020distributed}. 
% A near optimal distributed Min-Max data similarity (MMDS) algorithm is proposed in \cite{beznosikovetal2020distsaddle} for saddle point problems with a suitable data similarity assumption. 
%%MMDS is based on full batch gradient computations and requires solving an inner saddle point problem at every iteration. MMDS allows for communication efficiency by choosing only one node uniformly at random to update the iterates. However, every node computes the full batch gradient before heading to next gradient based updates. Moreover, this scheme employs accelerated gossip \cite{liu2011accelerated} multiple times to propagate the gradients and model updates to the entire network. Communication complexity of MMDS is shown to depend on eigengap of weight matrix $W$, while gradient computation complexity is not investigated.
%Decentralized parallel optimistic stochastic gradient method (DPOSG) was proposed in \cite{liu2020decentralized} for nonconvex-nonconcave saddle point problems. 
%%This method involves local model averaging step (multiple communication rounds) to reduce the effect of consensus error. 
%A gradient tracking based algorithm called DMHSGD for solving nonconvex-strongly concave saddle point problems is proposed in \cite{xianetal2021fasterdecentnoncvxsp}.
%%, uses a large mini-batch at the first iteration and requires the nodes to communicate multiple times to share both model and gradient updates. 
%A detailed discussion on related work is provided in Appendix \ref{related_work_appendix}. Table \ref{ratetable} positions our work in the context of existing methods.  
%\mynote{PB: rates? Extra step?}
%

%\vspace{-0.05in}
%\begin{table}[!h]\scriptsize
%%	\caption{Comparison of proposed optimization algorithms for decentralized saddle point problems with state-of-the-art algorithms based on optimistic gradient descent ascent and gradient tracking schemes. SGO stand for Stochastic Gradient Oracle .} 
%	\caption{Comparison of proposed optimization algorithms for decentralized saddle point problems with state-of-the-art algorithms. SGO and VR denote respectively Stochastic Gradient Oracle and Variance Reduction. Abbreviations SC-SC, C-C, NC-NC respectively stands for Strongly convex-Strongly concave, Convex-Concave, Nonconvex-Nonconcave } 
%			\vspace{-0.1in}
%	\label{ratetable}
%	\begin{center}
%		%		\setlength\extrarowheight{-1pt}
%		%setlength{\tabcolsep}{0.4mm}
%		\begin{tabular}{ccccccccc}
%			\hline
%		&	\textbf{Algorithm} & \textbf{SGO} & \textbf{VR} &  \textbf{Non-smooth} & \textbf{Gossip} & \textbf{Type of } & \textbf{Computation} & \textbf{Communication}  \\ 
%		&	&   &  & \textbf{case} & \textbf{step} & \textbf{functions} & \textbf{complexity} & \textbf{complexity}  \\
%			\hline
%		& & & & & & & & \\
%		\multirow{8}{*}{ \begin{turn}{90} \textbf{Without Compression} \end{turn} } & & & & & & & & \\
%		\cline{3-8}
%		& MMDS \cite{beznosikovetal2020distsaddle}  & \xmark &  \xmark & \xmark & \cmark & SC-SC & - & $\tilde{\mathcal{O}}( \log^2(\frac{1}{\epsilon}) )$ \\
%		\cline{3-8}
%		& DMHSGD \cite{xianetal2021fasterdecentnoncvxsp} & \cmark & \xmark & \xmark & \xmark & NC-SC & $\mathcal{O}(\frac{\kappa^3}{(1-\lambda_2(W))^2\epsilon^{3}} )$ & $\mathcal{O}(\frac{\kappa^3}{(1-\lambda_2(W))^2\epsilon^{3}} )$	\\ 
%	 \cline{3-8}
%		& DES \cite{beznosikov2020distributed} & \cmark & \xmark &  \xmark & \cmark & SC-SC & $\tilde{\mathcal{O}}( \frac{\kappa_f^2}{L^2\epsilon} )$ & $\tilde{\mathcal{O}}( \kappa_f \sqrt{\kappa}_g \log(1/\epsilon ) )$ \\
%%			 & & & & & & & \\
%	\hline
%	& DPOSG \cite{liu2020decentralized} & \cmark & \xmark & \xmark & \cmark & NC-NC & $\mathcal{O}(\frac{1}{\epsilon^{12}})$ & $\tilde{\mathcal{O}}( \frac{1}{\epsilon^{12}} )$ \\
%& & & & & & & & \\
%	\hline
%&	GT-EG \cite{mukherjeecharaborty2020decentralizedsaddle} & \xmark & \xmark & \xmark & \xmark & SC-SC & $\mathcal{O}\left(\kappa_f^{4/3} \log\left(\frac{1}{\epsilon} \right)\right)$ & $\mathcal{O}\left(\kappa_f^{4/3} \log\left(\frac{1}{\epsilon} \right)\right)$ \\
%& &  & & & & & \\
%	\hline
%&	DSPAwLA\cite{nunezcortes2017distsaddlesubgrad}  & \xmark & \xmark & \cmark & \xmark & C-C & $\mathcal{O}(1/\epsilon^2)$ & $\mathcal{O}(1/\epsilon^2)$ \\
%	\hline
%&	{\color{blue}{C-RDPSG}} & \cmark & \xmark & \cmark & \xmark & SC-SC & $\mathcal{O}(\frac{\kappa_f^2 \kappa^2_g}{L^2\epsilon} )$ & $\mathcal{O}(\frac{\kappa_f^2 \kappa^2_g}{\epsilon} )$ \\
%&	\textbf{(Theorem \ref{thm:complexity_general_stoch})} & & & & & & \\
%	\hline
%&	{\color{blue}{C-DPSVRG}}  & \xmark & \cmark &  \cmark & \xmark & SC-SC & $\mathcal{O}(\max \{\kappa_f^2, \kappa_g \} \log( \frac{1}{\epsilon} ) )$ & $\mathcal{O}(\max \{\kappa_f^2, \kappa_g \} \log( \frac{1}{\epsilon} ) ) $ \\
%&	\textbf{(Theorem \ref{thm:svrg_complexity})}  & & & & & & \\
%	\hline
%&	& & & & & & & \\
%%		& \multicolumn{6}{c}{\textbf{With Compression}}  \\
%%		& & & & & & & \\
%%		\hline
%% 	{\color{blue}{C-RDPSG}} & \cmark & \xmark & \cmark & \xmark & SC-SC & $\mathcal{O}(\frac{(1+\delta)^4\kappa_f^2 \kappa^2_g}{L^2\epsilon} )$ & $\mathcal{O}(\frac{(1+\delta)^4\kappa_f^2 \kappa^2_g}{\epsilon} )$ \\
%% \textbf{(Theorem \ref{thm:complexity_general_stoch})} & & & & & & \\
%% \hline
%% {\color{blue}{C-DPSVRG}}  & \xmark & \cmark &  \cmark & \xmark & SC-SC & $\mathcal{O}((1+\delta)$ & $\mathcal{O}((1+\delta)$ \\
%% & & & & & & $\max \{\kappa_f^2, \kappa_g, \sqrt{\delta}\kappa_f^2 \kappa_g \} \log( \frac{1}{\epsilon} ) )$ & $\max \{\kappa_f^2, \kappa_g, \sqrt{\delta}\kappa_f^2 \kappa_g \} \log( \frac{1}{\epsilon} ) )$ \\
%% \hline 
%% \textbf{(Theorem \ref{thm:svrg_complexity})}  & & & & & & \\
%% \hline
%% 	{\color{blue}{C-RDPSG}} & \xmark & \xmark & \cmark & \xmark & SC-SC & $\mathcal{O}((1+\delta)^2\kappa_f^2 \kappa_g )\log\left(\frac{1}{\epsilon}\right)$ & $\mathcal{O}((1+\delta)^2\kappa_f^2 \kappa_g )\log\left(\frac{1}{\epsilon}\right)$ \\
%% \textbf{(Theorem \ref{thm:complexity_deterministic_IPDHG})} & & & & & & \\
% \hline
%		\end{tabular}
%	\end{center}
%\end{table}
%\resizeableyellownote{2.5}{1.5}{ Compression + Gossip schemes not explored yet}

%\specialrule{line width}{above space}{below space}

